Keypoint Transformer: Solving Joint Identification in Challenging Hands and Object Interactions for Accurate 3D Pose Estimation

We propose a robust and accurate method for estimating the 3D poses of two hands in close interaction from a single color image. This is a very challenging problem, as large occlusions and many confusions between the joints may happen. State-of-the-art methods solve this problem by regressing a heatmap for each joint, which requires solving two problems simultaneously: localizing the joints and recognizing them. In this work, we propose to separate these tasks by relying on a CNN to first localize joints as 2D keypoints, and on self-attention between the CNN features at these keypoints to associate them with the corresponding hand joint. The resulting architecture, which we call "Keypoint Transformer", is highly efficient as it achieves state-of-the-art performance with roughly half the number of model parameters on the InterHand2.6M dataset. We also show it can be easily extended to estimate the 3D pose of an object manipulated by one or two hands with high performance. Moreover, we created a new dataset of more than 75,000 images of two hands manipulating an object fully annotated in 3D and will make it publicly available.

==> 3b_hand_pose_repr.tex <==
\subsection{Hand Pose Representations and Losses}
\label{sec:pose_rep_loss}

\vincentrmk{Since we need space, we can move this to the supp mat. Keep the subsection but only to point to the supp mat after mentioning we consider 3 representations, each with a suitable loss}


\vincent{We consider three main hand pose representations: 3D joint locations, 2.5D~\cite{umar, Moon_2020_ECCV_InterHand2.6M} joint locations, and MANO joint angles~\cite{Romero2017EmbodiedH}, $\theta$.} Previous methods relying on CNN architectures~\cite{hasson20_handobjectconsist, Angjoo, Pavlakos2018LearningTE, Pavlakos2019TexturePoseSH, hasson19_obman} have noted that regressing model parameters such as joint angles is less accurate (in terms of joint error) than regressing the joint locations directly. However, regressing MANO joint angles provides access to the complete hand mesh required for modeling contacts and interpenetration during interactions~\cite{Taheri2020GRABAD, Brahmbhatt2020ContactPoseAD, hasson19_obman} or for learning in a weakly supervised setup~\cite{Kulon2020WeaklySupervisedMH,Baek2020WeaklySupervisedDA,hasson20_handobjectconsist}, which could be interesting for future extension of our method. As we show later in our experiments, the Keypoint Transformer enables MANO joint angle representation to achieve competitive performance when compared to the joint location representation. \vincent{We detail the three possible representations below. Their respective losses are summarized in Table~\ref{tab:pose_loss}. }


% As noted in previous works~\cite{hasson20_handobjectconsist, Angjoo, Pavlakos2018LearningTE, Pavlakos2019TexturePoseSH, hasson19_obman}, regressing 3D joint locations directly is more accurate (in terms of joint error) than regressing model parameters such as the MANO joint angles. However, regressing MANO joint angles provides access to the complete hand mesh required for modeling contacts and interpenetration during interactions~\cite{Taheri2020GRABAD, Brahmbhatt2020ContactPoseAD, hasson19_obman} or for learning in a weakly supervised setup~\cite{Kulon2020WeaklySupervisedMH,Baek2020WeaklySupervisedDA,hasson20_handobjectconsist}, which could be interesting for future extension of our method. We therefore consider both options (3D joint locations and joint angles) as outputs and show later in our experiments that our architecture enables joint angle representation to achieve competitive performance when compared to the joint location representation. For the 3D joint hand locations, we consider two types of representations: parent-relative joint vectors and parent-relative 2.5D pose.  We detail the three possible representations and their corresponding losses below. 


% \vspace{-12px}



\paragraph{3D representation.}  In this representation, each joint $j$ is associated with a parent-relative joint vector $V(j) = J_\ThD(j) - J_\ThD(p(j))$, where $J_\ThD$ is the 3D joint location and $p(j)$ refers to the parent joint index of joint $j$. We estimate 20 joint vectors per hand using 20 joint queries (40 queries for two hands), from which we can compute the root-relative 3D location, $J_{3D}^r$ of each joint by simple  accumulation. The advantage of this representation is that it defines the hand pose relative to its root without requiring knowledge of the camera intrinsics.

% When using this representation, we supervise our architecture using a pose loss $\calL_\pose^V$ that combines 2 loss terms:
% %
% \begin{equation}
% \calL_\pose^V = \calL_\calV + \calL_\ThD\> , 
% \label{eq:L_pose_V}
% \end{equation}
% %
% where $\calL_\calV$ is the L1 loss between the predicted joint vectors and their ground truth, $\calL_\ThD$ is the L1 loss between the  root-relative 3D joint locations retrieved by summing the predicted joint vectors and their ground truth.

% \vspace{-12px}

\paragraph{2.5D representation~\cite{umar, Moon_2020_ECCV_InterHand2.6M}.} 

In this representation, each joint is parameterised by its 2D location $J_\TwD$, and the difference $\Delta Z^p$ between its  depth and the depth of its parent joint. The camera intrinsics matrix $K$ and the absolute depth $Z_\text{root}$ of the root joint (the wrist)~\cite{Moon_2020_ECCV_InterHand2.6M} or the scale of the hand~\cite{umar} are then required to reconstruct the 3D pose of the hand in camera coordinate system as $J_\ThD = K^{-1} \cdot (Z_\text{root}+\Delta Z^r) \cdot  \big[J_{\TwD_x},J_{\TwD_y},1\big]^T \>,$
where $\Delta Z^r$ is the root-relative depth of the joint computed from its predicted $\Delta Z^p$ and the predicted $\Delta Z^p$ for its parents. $J_{\TwD_x}, J_{\TwD_y}$ are the predicted $x$ and $y$ coordinates of $J_\TwD$. 

When using this representation, we also predict the root depth $Z_\text{root}$ separately using RootNet~\cite{Moon2019CameraDT} as in \cite{Moon_2020_ECCV_InterHand2.6M}. Each joint query estimates the $J_{\TwD}$ and $\Delta Z^r$ for that joint and we require a total of 21 joint queries (42 for two hands) to estimate the 2.5D pose per hand. 

% We supervise our architecture using a pose loss $\calL_\pose^\text{2.5D}$ that combines two loss terms:
% %
% \begin{equation}
% \calL_\pose^\text{2.5D} = \calL'_\TwD + \calL_Z \> , 
% \label{eq:L_pose_25D}
% \end{equation}
% %
% where $\calL'_\TwD$ is the L1 loss between the predicted 2D locations of the joints and their ground truth, $\calL_Z$ is the L1 loss between the predicted $\Delta Z^p$ and their ground truth.

% \vspace{-12px}

\paragraph{MANO joint angles, $\theta$~\cite{Romero2017EmbodiedH}.} 
In this representation, each 3D hand pose is represented by 16 3D joint angles in the hand kinematic tree and is estimated using 16 joint queries per hand. The MANO hand shape parameter is estimated along with the relative translation between the hands using an additional query. Given the predicted 3D joint angles $\theta$ for each hand and the shape parameters $\beta$, it is possible to compute the root-relative 3D joint locations, $J_{3D}^r$ of each hand.


\begin{table}
    \centering
    \scalebox{0.8}{
    \begin{tabular}{@{}P{2.0cm}P{8.0cm}@{}}
    \toprule
    Representation & $\calL_{hand-pose}$ \\
    \midrule
    3D & $\sum_j \lvert\lvert V(j) - V(j)^*\lvert\lvert_1 + \sum_j \lvert\lvert J_{3D}^r(j) - J_{3D}^{r^*}(j)\lvert\lvert_1$\\
    2.5D & $\sum_j \lvert\lvert J_{2D}(j) - J_{2D}^*(j)\lvert\lvert_1 + \sum_j \lvert\Delta Z^r(j) - \Delta Z^{r^*}(j) \lvert$\\
    $\theta$ & $\sum_j \lvert\lvert J_{3D}^r(j) - J_{3D}^{r^*}(j)\lvert\lvert_1 + \sum_j \lvert\lvert \theta (j) - \theta^* (j) \lvert\lvert_1$\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-5px}
    \caption{Hand pose losses for different pose representations. $x^*$ denotes the ground-truth values for variable $x$ and $x(j)$ the value of $x$ at joint $j$.
}
    \vspace{-12px}
    \label{tab:pose_loss}
\end{table}


\paragraph{Implementation details}
The encoder of our U-Net~\cite{unet} is based on ResNet-50~\cite{He2016DeepRL} architecture while a series of upsampling and convolutional layers with skip connections forms the U-Net decoder. We use 256$\times$256 pixels as input image resolution, 128$\times$128 pixels as heatmap resolution, and 
$\sigma=1.25$.

\vincentrmk{move this to the supp mat: }
depending on the output representation as discussed in Tab.~\ref{tab:pose_loss}. The keypoint detector is pretrained before training the entire network end-to-end.
% During the initial few epochs when the estimated keypoint heatmap is less accurate, we use the ground truth 3D joint reprojections and ground truth object segmentations for obtaining keypoint locations and later switch to the predicted heatmap and segmentations.
We use a 256$\times$256 pixel image patch loosely cropped around the hand and object as input to the network and use the Adam~\cite{KingmaB14} optimizer with a learning rate of $\text{10}^\text{-4}$ and $\text{10}^\text{-5}$ for the attention modules and CNN backbone, respectively. We train the network for 50 epochs on 3 Titan V GPUs with a total batch size of 78 and use on-line augmentation techniques such as rotation, scale and mirroring during training.

% DO NOT DELETE THIS
% Mean obj adi corner error 025_mug (count = 2092) = 0.073008 mts
% Mean obj adi corner error 011_banana (count = 154) = 0.109071 mts
% Mean obj adi corner error 019_pitcher_base (count = 900) = 0.072770 mts
% Mean obj adi corner error 024_bowl (count = 839) = 0.082044 mts
% Mean obj adi corner error 037_scissors (count = 22) = 0.065035 mts
% Mean obj adi corner error 035_power_drill (count = 343) = 0.072891 mts
% Mean obj corner adi all = 0.076069 mts

==> ablation.tex <==

\section{Ablation Study}

\paragraph{Comparison with CNN architecture}

As we show in Table~\ref{tab:interhand}, our CNN-Transformer architecture outperforms the CNN-only architecture of \cite{Moon_2020_ECCV_InterHand2.6M} by a large margin~(16\%). The explicit modeling of the relationship between the image features at only keypoint locations allows our architecture to attain better accuracy. %In our architecture, we employ a CNN to only localize the joints in the image and utilize the features relationship modeling capabilities of the Transformer to recognize the joints and predict their 3-D locations.
\vspace{-12px}
\paragraph{Visualization of attention}

To understand which features of the encoder are attended by a given joint query at the decoder, we visualize the cross-attention weights for three joint queries of the right hand in Fig.~\ref{fig:attn}.  The joint queries learn to attend to the keypoint features that mostly correspond to the respective joint location in the image. %In other words, for each joint query, the decoder selects the image features from keypoint locations that correspond to the respective joint and estimates joint-related pose parameters such as joint angle and joint vector.


%% \paragraph{Transformer vs CNN}
%% \vincentrmk{Mention again the comparison with the facebook baseline}


%% \paragraph{Visualization of attention}
%% In order to understand which features of the encoder are considered for a given joint query to the decoder, we visualize the cross-attention weights for three joint queries of the right hand: Index finger tip joint, middle finger PIP joint and pinky finger MCP joint in Figure~\ref{fig:attn}. The joint queries learn to attend to the encoder features that only belong to the respective joint location in the image. In other words, for each joint query the decoder selects the image features from keypoint locations that correspond to the respective joint and estimates joint-related pose parameters such as joint angle and joint vector.

%% \begin{figure}

\begin{figure}[]
\begin{center}
\includegraphics[trim=50 120 20 120,clip, width=1.0\linewidth]{figures/ablation/attn.pdf} 
\end{center}
\vspace{-0.35cm}
\caption{{\bf Visualizing the cross-attention for three joint queries of the right hand:} Index fingertip (red), middle PIP (blue) and pinky MCP joints (yellow). For each joint query, the corresponding colored circles in the third image indicates the locations of the keypoints attended by the query. The radius of the circle is proportional to the attention weight. We observe that each joint query select image features from the respective joint location.}% For each joint query, the decoder selects the image features only from the location of the joint and estimates joint-related pose parameters such as joint angle and joint vector.}
% \sayanrmk{TODO: Change Font Of Fig}}
\label{fig:attn}
\vspace{-0.3cm}
\end{figure}
\vspace{-12px}
\paragraph{How important is the keypoint identity loss?}
Table~\ref{tab:ablation} (`Ours w/o $\calL_\text{KI}$') shows the effect of not using the keypoint identity prediction loss in the transformer encoder. This loss helps the architecture to not confuse the joints and results in 20\% higher accuracy.

% We study the effect of not minimizing the keypoint identity prediction loss of Section~\ref{sec:ki_loss} on the encoder in Table~\ref{tab:ablation} (`Ours w/o $\calL_\text{KI}$') using the InterHand2.6M dataset. The keypoint identity loss improves the pose accuracy of the interacting hands by $\mathtt{\sim}$4mm or 17\%. It also improves the relative hand translation accuracy by a large margin~(13~mm). As noted in Figure~\ref{fig:attn}, a joint query in the decoder attends to the encoder features that correspond to the respective joint. The external supervision provided by the keypoint identity prediction loss makes the encoder features more joint aware allowing the decoder to query and select features of the particular joint more efficiently.


% \begin{table}[]
%     \centering
%     \scalebox{0.8}
% 	     {
%     \begin{tabular}{l|c|c|c|c }
%     \multirow{2}{*}{\parbox{1.4cm}{\centering Joint Association}} & \multicolumn{3}{c |}{\centering MPJPE (mm)} & {\centering MRRPE(mm)}  \\
%     & Single Hand & Inter. Hand & All &  \\
%     \hline
%     No & 14.63 & 22.25 & 18.47 & 46.81 \\
%     Yes & 12.42 & 17.08 & 14.76 & 33.14 \\
    
%     \end{tabular}}
%     \vspace{0.1cm}
%     \caption{Effect of the keypoint identity prediction loss in the Tranformer encoder on InterHand2.6M. The keypoint-joint association guides the Transformer in selecting more appropriate features from the encoder, resulting in higher accuracy of the pose estimates especially during close hand interactions.}
%     \label{tab:joint_ablation}
%     % \vspace{-0.7cm}
% \end{table}

\vspace{-12px}
\paragraph{How important is multi-scale feature sampling?}
In Table~\ref{tab:ablation}, we compare our method with a DETR~\cite{detr}-style architecture which uses low-resolution feature map at the last layer of U-Net encoder as input tokens to the transformer. More details about this architecture are provided in the supplementary material. Our architecture which uses multi-scale feature map sampling achieves 18\% higher accuracy.

% To understand the importance of multi-scale feature sampling, we evaluate the performance of a DETR~\cite{detr} style architecture which provides low-resolution feature maps from a CNN backbone as input tokens to the transformer encoder-decoder architecture. For fair comparison, the transformer architecture is identical to the one used in our method. More implementation details are provided in the suppl.mat.

% Table~\ref{tab:ablation} compares the accuracy of the DETR-style architecture with our architecture on InterHand2.6M when predicting hand poses with the joint vector representation as output. Our architecture is $\mathtt{\sim}$4~mm more accurate on interacting hands and 18\% more accurate overall. It also predicts more accurate relative translation between the hands. Note that the computational complexity between DETR-style architecture and ours is similar except for the additional U-net decoder in our method. 

\begin{table}[]
    \centering
    \scalebox{0.8}
	     {
    \begin{tabular}{l|c| c| c|c }
    & \multicolumn{3}{c |}{\centering MPJPE (mm)} & {\centering MRRPE(mm)}  \\
    & Single Hand & Inter. Hand & All &  \\
    \hline
    Ours w/o $\calL_\text{KI}$ & 14.63 & 22.25 & 18.47 & 46.81 \\
    DETR~\cite{detr}-style & 15.25 & 20.86 & 18.07 & 39.08\\
    Ours & 12.42 & 17.08 & 14.76 & 33.14 \\
    
    \end{tabular}}
    \vspace{0.1cm}
    \caption{\textbf{Ablation study on InterHand2.6M.} The keypoint identity loss $\calL_\text{KI}$ increases the accuracy of pose estimation by 20\%. The DETR~\cite{detr}-style architecture uses features only from the last layer of the U-Net encoder, which is a low-resolution feature map, resulting in inferior performance.}
    % \caption{Effect of multi-scale feature sampling on InterHand2.6M. The DETR~\cite{detr}-style architecture uses features only from the last layer of the U-net encoder, which is a low-resolution feature map. Our architecture samples multi-scale features from different layers of the U-net decoder resulting in higher accuracy of the pose estimates.}
    \label{tab:ablation}
    \vspace{-0.5cm}
\end{table}

